csa2sls: A complete subset approach for many instruments using Stata

We develop a Stata command $\texttt{csa2sls}$ that implements the complete subset averaging two-stage least squares (CSA2SLS) estimator in Lee and Shin (2021). The CSA2SLS estimator is an alternative to the two-stage least squares estimator that remedies the bias issue caused by many correlated instruments. We conduct Monte Carlo simulations and confirm that the CSA2SLS estimator reduces both the mean squared error and the estimation bias substantially when instruments are correlated. We illustrate the usage of $\texttt{csa2sls}$ in Stata by an empirical application.

==> old_files/BLP.log.tex <==
. set seed 2022
{\smallskip}
. insheet using "../data/BLP.csv", comma clear
(54 vars, 2,217 obs)
{\smallskip}
. csa2sls y hpwt air mpd space (price = sumother1 sumotherhpwt sumotherair ///
> sumothermpd sumotherspace sumrival1 sumrivalhpwt sumrivalair sumrivalmpd ///
> sumrivalspace)
 
 
Complete Subset Model Averaging 2SLS  Regression     Number of obs = 2217
                                                     Number of IVs = 10
                                                     Root MSE      = 1.1244518
 
 
\HLI{13}{\TOPT}\HLI{64}
           y {\VBAR}      Coef.   Std. Err.      z    P>|z|     [95\% Conf. Interval]
\HLI{13}{\PLUS}\HLI{64}
       price {\VBAR}   -.142563   .0117095   -12.18   0.000    -.1655131   -.1196128
        hpwt {\VBAR}   1.422452    .414676     3.43   0.001     .6097024    2.235202
         air {\VBAR}   .5620958   .1379201     4.08   0.000     .2917772    .8324143
         mpd {\VBAR}   .1579617   .0471821     3.35   0.001     .0654864    .2504369
       space {\VBAR}   2.284253   .1289588    17.71   0.000     2.031499    2.537008
       _cons {\VBAR}  -2.342198   .2673599    -8.76   0.000    -2.866214   -1.818182
\HLI{13}{\BOTT}\HLI{64}
Instrumented : price 
Instruments : sumother1 sumotherhpwt sumotherair sumothermpd sumotherspace sumrival1 s
> umrivalhpwt sumrivalair sumrivalmpd sumrivalspace 
optimal k : 9
-------------------------------------------------------------------------------


==> old_files/Yogo_14IVs.log.tex <==
. set seed 2022
{\smallskip}
. insheet using "../data/USAQ_extend.csv", comma clear
(23 vars, 206 obs)
{\smallskip}
. csa2sls dc (rrf = z1-z14)
 
 
Complete Subset Model Averaging 2SLS Regression      Number of obs = 206
                                                     Number of IVs = 14
                                                     Root MSE      = .00551145
 
 
\HLI{13}{\TOPT}\HLI{64}
          dc {\VBAR}      Coef.   Std. Err.      z    P>|z|     [95\% Conf. Interval]
\HLI{13}{\PLUS}\HLI{64}
         rrf {\VBAR}  -.0650585   .1167877    -0.56   0.577    -.2939582    .1638413
       _cons {\VBAR}   .0051027   .0005265     9.69   0.000     .0040707    .0061348
\HLI{13}{\BOTT}\HLI{64}
Instrumented : rrf 
Instruments  : z1 z2 z3 z4 z5 z6 z7 z8 z9 z10 z11 z12 z13 z14 
optimal k    : 1
\HLI{78}


==> old_files/Yogo_4IVs.log.tex <==
. set seed 2022
{\smallskip}
. insheet using "../data/USAQ.csv", comma clear
(12 vars, 206 obs)
{\smallskip}
. csa2sls dc (rrf = z1-z4)
 
 
Complete Subset Model Averaging 2SLS Regression      Number of obs = 206
                                                     Number of IVs = 4
                                                     Root MSE      = .00539602
 
 
\HLI{13}{\TOPT}\HLI{64}
          dc {\VBAR}      Coef.   Std. Err.      z    P>|z|     [95\% Conf. Interval]
\HLI{13}{\PLUS}\HLI{64}
         rrf {\VBAR}  -.0247716   .1169836    -0.21   0.832    -.2540552     .204512
       _cons {\VBAR}   .0050118   .0005219     9.60   0.000     .0039888    .0060348
\HLI{13}{\BOTT}\HLI{64}
Instrumented : rrf 
Instruments  : z1 z2 z3 z4 
optimal k    : 1
\HLI{78}


==> stata.tex <==

\section{User's guide to stata.sty}

\texttt{stata.sty} is a {\LaTeX} package containing macros and environments to
help authors produce documents containing {\stata} output and syntax
diagrams.

\subsection{Citing the Stata manuals}

The macros for generating references to the {\stata} manuals are
given in table~\ref{table:manref}.

\clearpage
\begin{table}[h!]
\caption{Stata manual references}
\label{table:manref}
\begin{center}
\begin{tabular}{ll}
\hline
\noalign{\smallskip}
Example & Result\\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\verb+\dref{merge}+ & \dref{merge}\\
\verb+\grefa{graph editor}+ & \grefa{graph editor}\\
\verb+\grefb{graph}+ & \grefb{graph}\\
\verb+\grefci{line\_options}+ & \grefci{line\_options}\\
\verb+\grefdi{connectstyle}+ & \grefdi{connectstyle}\\
\verb+\iref{data types}+ & \iref{data types}\\
\verb+\mreff{intro}+ & \mreff{intro}\\
\verb+\mrefa{ado}+ & \mrefa{ado}\\
\verb+\mrefb{declarations}+ & \mrefb{declarations}\\
\verb+\mrefc{mata clear}+ & \mrefc{mata clear}\\
\verb+\mrefd{matrix}+ & \mrefd{matrix}\\
\verb+\mrefe{st\_view($\,$)}+ & \mrefe{st\_view($\,$)}\\
\verb+\mrefg{Glossary}+ & \mrefg{Glossary}\\
\verb+\miref{mi impute}+ & \miref{mi impute}\\
\verb+\mvref{cluster}+ & \mvref{cluster}\\
\verb+\pref{syntax}+ & \pref{syntax}\\
\verb+\rref{regress}+ & \rref{regress}\\
\verb+\stref{streg}+ & \stref{streg}\\
\verb+\svyref{svy:~tabulate oneway}+ & \svyref{svy:~tabulate oneway}\\
\verb+\tsref{arima}+ & \tsref{arima}\\
\verb+\uref{1~Read this---it will help}+ & \uref{1~Read this---it will help}\\
\verb+\xtref{xtreg}+ & \xtref{xtreg}\\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Stata syntax}

Here is an example syntax display:

\begin{stsyntax}
\dunderbar{reg}ress
    \depvar\
    \optindepvars\
    \optif\
    \optin\
    \optweight\
    \optional{,
    \underbar{noc}onstant
    \underbar{h}ascons
    tsscons
    vce({\it vcetype\/})
    \underbar{l}evel(\num)
    \underbar{b}eta
    \underbar{ef}orm(\ststring)
    \underbar{nohe}ader
    plus
    \dunderbar{dep}name(\varname)
    mse1}
\end{stsyntax}

\noindent
This syntax is generated by

\begin{stverbatim}
\begin{verbatim}
\begin{stsyntax}
\dunderbar{reg}ress
    \depvar\
    \optindepvars\
    \optif\
    \optin\
    \optweight\
    \optional{,
    \underbar{noc}onstant
    \underbar{h}ascons
    tsscons
    vce({\it vcetype\/})
    \underbar{l}evel(\num)
    \underbar{b}eta
    \underbar{ef}orm(\ststring)
    \underbar{nohe}ader
    plus
    \dunderbar{dep}name(\varname)
    mse1}
\end{stsyntax}
\end{verbatim}
\end{stverbatim}

\noindent
Each command should be formatted using a separate \texttt{stsyntax}
environment.  Table~\ref{table:syntax} contains an example of each syntax
macro provided in \texttt{stata.sty}. 

\begin{table}[h!]
\caption{\stata{} syntax elements}
\label{table:syntax}
\fontsize{10}{14}\selectfont
\begin{center}
\begin{tabular}{ll@{\hspace{.5in}}ll}
\noalign{\smallskip}
\hline
\noalign{\smallskip}
Macro & Result
&
Macro & Result
\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\verb+\LB+ & \LB
&
\verb+\ifexp+ & \ifexp
\\
\noalign{\smallskip}
\verb+\RB+ & \RB
&
\verb+\optif+ & \optif
\\
\noalign{\smallskip}
\verb+\varname+ & \varname
&
\verb+\inrange+ & \inrange
\\
\noalign{\smallskip}
\verb+\optvarname+ & \optvarname
&
\verb+\optin+ & \optin
\\
\noalign{\smallskip}
\verb+\varlist+ & \varlist
&
\verb+\eqexp+ & \eqexp
\\
\noalign{\smallskip}
\verb+\optvarlist+ & \optvarlist
&
\verb+\opteqexp+ & \opteqexp
\\
\noalign{\smallskip}
\verb+\newvarname+ & \newvarname
&
\verb+\byvarlist+ & \byvarlist
\\
\noalign{\smallskip}
\verb+\optnewvarname+ & \optnewvarname
&
\verb+\optby+ & \optby
\\
\noalign{\smallskip}
\verb+\newvarlist+ & \newvarlist
&
\verb+\optional{text}+ & \optional{text}
\\
\noalign{\smallskip}
\verb+\optnewvarlist+ & \optnewvarlist
&
\verb+\optweight+ & \optweight
\\
\noalign{\smallskip}
\verb+\depvar+ & \depvar
&
\verb+\num+ & \num
\\
\noalign{\smallskip}
\verb+\optindepvars+ & \optindepvars
&
\verb+\ststring+ & \ststring
\\
\noalign{\smallskip}
\verb+\opttype+ & \opttype
\\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\end{table}

\verb+\underbar+ is a standard macro that generates underlines.  The
\verb+\dunderbar+ macro from \texttt{stata.sty} generates the underlines for
words with descenders. For example,

\begin{itemize}
\item
\verb+{\tt \underbar{reg}ress}+ generates {\tt \underbar{reg}ress}

\item
\verb+{\tt \dunderbar{reg}ress}+ generates {\tt \dunderbar{reg}ress}

\end{itemize}

The plain \TeX{} macros \verb+\it+, \verb+\sl+, and \verb+\tt+ are
also available. \verb+\it+ should be used to denote ``replaceable''
words, such as {\it varname}. \verb+\sl+ can be used for emphasis but
should not be overused. \verb+\tt+ should be used to denote words that
are to be typed, such as command names.

When describing the options of a new command, the \verb+\hangpara+ and
\verb+\morehang+ commands provide a means to reproduce a paragraph style
similar to that of the Stata reference manuals.  For example,

\hangpara
{\tt level(\num)} specifies the confidence level, as a percentage,
for confidence intervals.  The default is {\tt level(95)} or as set by {\tt
set level}; see \uref{20.7~Specifying the width of confidence intervals}.

\noindent
was generated by

\begin{stverbatim}
\begin{verbatim}
\hangpara
{\tt level(\num)} specifies the confidence level, as a percentage,
for confidence intervals.  The default is {\tt level(95)} or as set by {\tt
set level}; see \uref{20.7~Specifying the width of confidence intervals}.
\end{verbatim}
\end{stverbatim}


\subsection{Stata output}
\label{sec:output}

When submitting {\sl Stata Journal\/} articles that contain {\stata} output,
also submit a do-file and all relevant datasets that reproduce the output
(do not forget to set the random-number seed when doing simulations).  The
following is an example of the \texttt{stlog} environment containing output
from simple linear regression analysis on two variables in {\tt auto.dta}:

\begin{stlog}
\input{output1.log.tex}\nullskip
\end{stlog}

\noindent
The above listing was included using

\begin{stverbatim}
\begin{verbatim}
\begin{stlog}
\input{output1.log.tex}\nullskip
\end{stlog}
\end{verbatim}
\end{stverbatim}

\noindent
where \texttt{output1.log.tex} is a Stata log file converted to include \TeX{}
macros by using the \stcmd{sjlog} command (more on \stcmd{sjlog} shortly).
\verb+\nullskip+ adjusts the spacing around the log file.

\clearpage
On occasion, it is convenient (maybe even necessary) to be able to omit some of
the output or let it spill onto the next page.  Here is a listing containing
the details of the following discussion:

\begin{stverbatim}
\begin{verbatim}
\begin{stlog}
. sysuse auto
(1978 Automobile Data)
{\smallskip}
. regress mpg weight
{\smallskip}
\oom
{\smallskip}
\clearpage
\end{stlog}
\end{verbatim}
\end{stverbatim}

The \verb+\oom+ macro creates
a short message indicating omitted output in the following example, and the
\verb+\clearpage+ macro inserts a page break.

\begin{stlog}
. sysuse auto
(1978 Automobile Data)
{\smallskip}
. regress mpg weight
{\smallskip}
\oom
{\smallskip}
\clearpage
\end{stlog}

The output in \texttt{output1.log.tex} was generated from the following
\texttt{output.do}:

\begin{stlog}
\input{output.do.log.tex}
\end{stlog}

\noindent
\texttt{output.do} generates a \stcmd{.smcl} file, \stcmd{.log} file,
and \stcmd{.log.tex} file using \stcmd{sjlog}.  The actual file used in the
above listing was generated by

\begin{stlog}
. stlog type output.do
\end{stlog}

\texttt{sjlog.ado} is provided in the Stata package for \stcmd{sjlatex}.
\stcmd{sjlog} is a Stata command that helps generate log output to be included
in {\LaTeX} documents using the \texttt{stlog} environment.  If you have
installed the \stcmd{sjlatex} package, see the help file for \stcmd{sjlog} for
more details.  The lines that make up the table output from \stcmd{regress}
are generated from line-drawing macros defined in \texttt{stata.sty}; these
were macros written using some font metrics defined in \citet{texbook}.

By default, \texttt{stlog} sets an 8-point font for the log.  Use the
\texttt{auto} option to turn this behavior off, allowing you to use the
current font size, or change it by using\\ \verb+\fontsize{#}{#}\selectfont+.
The call to \texttt{stlog} with the \texttt{auto} option looks like
\verb+\begin[auto]{stlog}+.

Here is an example where we are using a 12-point font.

\vspace{-.2in}
{\fontsize{12}{13}\selectfont
\begin{stlog}[auto]
. stlog type output.do
\end{stlog}
}

\subsection{About tables}

Tables should be created using the standard \LaTeX{} methods.  See
\citet{latexbook} for a discussion and examples.

There are many user-written commands that produce \LaTeX{} output, including
tables.  Christopher F. Baum has written \stcmd{outtable}, a Stata command for
creating \LaTeX{} tables from Stata matrices.  Ben Jann's well-known
\stcmd{estout} command can also produce \LaTeX{} output.  To find other
user-written commands that produce \LaTeX{} output, try

\begin{stlog}
. net search latex
\end{stlog}
\clearpage

\subsubsection{Tables with notes}

Table~\ref{Table4} shows the order and format to use for notes to tables.



Order of notes should be
\vspace{-.08in}
\begin{enumerate}
\item source notes
\item notes applying to the whole table
\item notes applying to specific parts of the table
\item notes on significance levels
\end{enumerate}

Special notes:

\vspace{-.08in}
\begin{itemize}
\item Use \verb+\centering+ because the {\tt center} environment adds
unnecessary vertical spacing.

\item Place the \verb+\begin{threeparttable}+ line above the caption.

\end{itemize}


\subsection{Encapsulated PostScript (EPS)}

You can include figures by using either \verb+\includegraphics+ or
\verb+\epsfig+.

\begin{stverbatim}
\begin{verbatim}
\begin{figure}[h!]
\begin{center}
\includegraphics{eps/output1.eps}
\end{center}
\caption{Scatterplot with simple linear regression line}
\label{fig}
\end{figure}
\end{verbatim}
\end{stverbatim}

\begin{stverbatim}
\begin{verbatim}
\begin{figure}[h!]
\begin{center}
\epsfig{file=output1}
\end{center}
\caption{Scatterplot with simple linear regression line}
\label{fig}
\end{figure}
\end{verbatim}
\end{stverbatim}

Figure~\ref{fig} is included using \verb+\epsfig+ from the \texttt{epsfig}
package.  

\noindent
The graph was generated by running \texttt{output.do}, the
do-file given in section~\ref{sec:output}.  The \texttt{epsfig} package is
described in \citet*{latexcompanion}.

\begin{figure}[h!]
\begin{center}
\epsfig{file=output1}
\end{center}
\caption{Scatterplot with simple linear regression line}
\label{fig}
\end{figure}

\subsection{Stored results}

The \texttt{stresults} environment provides a table to describe the stored
results of a Stata command.  It consists of four columns: the first and third
column are for Stata result identifiers (for example, \stcmd{r(N)},
\stcmd{e(cmd)}), and the second and fourth columns are for a brief description
of the respective identifier.
%
Each group of results is generated using the \verb+\stresultsgroup+ macro.
%
The following is an example containing a brief description of the results that
\stcmd{regress} stored to \stcmd{e()}:

\begin{stresults}
\stresultsgroup{Scalars} \\
\stcmd{e(N)} & number of observations
&
\stcmd{e(F)} & $\scriptstyle F$ statistic
\\
\stcmd{e(mss)} & model sum of squares
&
\stcmd{e(rmse)} & root mean squared error
\\
\stcmd{e(df\_m)} & model degrees of freedom
&
\stcmd{e(ll\_r)} & log likelihood
\\
\stcmd{e(rss)} & residual sum of squares
&
\stcmd{e(ll\_r0)} & log likelihood, constant-only\\
\stcmd{e(df\_r)} & residual degrees of freedom
&
& \quad model \\
\stcmd{e(r2)} & $\scriptstyle R$-squared
&
\stcmd{e(N\_clust)} & number of clusters
\\
\stresultsgroup{Macros} \\
\stcmd{e(cmd)} & \stcmd{regress}
&
\stcmd{e(wexp)} & weight expression
\\
\stcmd{e(depvar)} & name of dependent variable
&
\stcmd{e(clustvar)} & name of cluster variable
\\
\stcmd{e(model)} & \stcmd{ols} or \stcmd{iv}
&
\stcmd{e(vcetype)} & title used to label Std.~Err.
\\
\stcmd{e(wtype)} & weight type
&
\stcmd{e(predict)} & program used to implement
\\
&&&\quad \stcmd{predict}
\\
\stresultsgroup{Matrices} \\
\stcmd{e(b)} & coefficient vector
&
\stcmd{e(V)} & variance--covariance matrix of
\\
&&&\quad the estimators\\
\stresultsgroup{Functions} \\
\stcmd{e(sample)} & marks estimation sample
\\
\end{stresults}

Alternatively, you can use the \texttt{stresults2} environment to create
a two column table.   This format works better if your descriptions are long.

\subsection{Examples and notes}

The following are environments for examples and notes similar to those
given in the Stata reference manuals.  They are generated using the
\texttt{stexample} and \texttt{sttech} environments, respectively.


\begin{stexample}
This is the default alignment for a \stata{} example.
\end{stexample}

\setlength{\stexamplehskip}{0pt}
\begin{stexample}
For this example, \verb+\stexamplehskip+ was set to
\texttt{\the\stexamplehskip}
before beginning.  This sentence is supposed to spill
over to the next line, thus revealing that the first sentence was indented.

This sentence is supposed to show that new paragraphs are automatically
indented (provided that \verb+\parindent+ is nonzero).
\end{stexample}

\begin{sttech}
For this note, \verb+\sttechhskip+ was set to \texttt{\the\sttechhskip}
(the default) before beginning.  This sentence is supposed to spill over to
the next line, thus revealing that the first sentence was indented.

This sentence is supposed to show that new paragraphs are automatically
indented (provided that \verb+\parindent+ is nonzero).
\end{sttech}

\subsection{Special characters}

Table \ref{table:specialch} contains macros that generate some useful
characters in the typewriter (fixed width) font.  The exceptions are
\verb+\stcaret+ and \verb+\sttilde+, which use the currently specified font;
the strictly fixed-width versions are \verb+\caret+ and \verb+\tytilde+,
respectively.

\begin{table}[h!]
\caption{Special characters}
\label{table:specialch}
\begin{center}
\begin{tabular}{ll@{\hspace{.5in}}ll}
\hline
\noalign{\smallskip}
Macro & Result &
Macro & Result \\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\verb+\stbackslash+ & \stbackslash
 &
\verb+\sttilde+ & \sttilde
\\
\verb+\stforslash+ & \stforslash 
&
\verb+\tytilde+ & \tytilde
\\
\verb+\stcaret+ & \stcaret
&
\verb+\lbr+ & \lbr
\\
\verb+\caret+ & \caret
&
\verb+\rbr+ & \rbr
\\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
\end{table}


\subsection{Equations and formulas}

In (\ref{eq:Exbar}), $\stbar{x}$ was generated using
\verb+\stbar{x}+.  Here \verb+\stbar+ is equivalent to the \TeX{} macro
\verb+\overline+.

\begin{equation}
E(\stbar{x}) = \mu
\label{eq:Exbar}
\end{equation}

In (\ref{eq:varbetahat}), $\sthat{\beta}$ was generated using
\verb+\sthat{\beta}+.  Here \verb+\sthat+ is equivalent to the \TeX{} macro
\verb+\widehat+.

\begin{equation}
V(\sthat{\beta}) = V\{(X'X)^{-1}X'y\} = (X'X)^{-1}X'V(y)X(X'X)^{-1}
\label{eq:varbetahat}
\end{equation}

\subsection{Other miscellaneous macros and environments}

The following box was created by

\begin{stverbatim}
\begin{verbatim}
\begin{ttbox}
A special framed
box that obeys lines and spaces.
\end{ttbox}
\end{verbatim}
\end{stverbatim}

\begin{ttbox}
A special framed
box that obeys lines and spaces.
\end{ttbox}

The following box was created by

\begin{stverbatim}
\begin{verbatim}
\ttboxWd=2.5in
\ttboxIndent=2em
\begin{ttbox}
Test that the width of the
box is \the\ttboxWd
and is indented \the\ttboxIndent
\end{ttbox}
\end{verbatim}
\end{stverbatim}

\ttboxWd=2.5in
\ttboxIndent=2em
\begin{ttbox}
Test that the width of the
box is \the\ttboxWd
and is indented \the\ttboxIndent
\end{ttbox}

\endinput

